Measurement of the $t\bar{t}$ production cross-section using $e\mu$ events with b-tagged jets in pp collisions at $\sqrt{s}$=13 TeV with the ATLAS detector

This paper describes a measurement of the inclusive top quark pair production cross-section ($\sigma_{t\bar{t}}$) with a data sample of 3.2 fb$^{-1}$ of proton--proton collisions at a centre-of-mass energy of $\sqrt{s}$=13 TeV, collected in 2015 by the ATLAS detector at the LHC. This measurement uses events with an opposite-charge electron--muon pair in the final state. Jets containing $b$-quarks are tagged using an algorithm based on track impact parameters and reconstructed secondary vertices. The numbers of events with exactly one and exactly two $b$-tagged jets are counted and used to determine simultaneously $\sigma_{t\bar{t}}$ and the efficiency to reconstruct and $b$-tag a jet from a top quark decay, thereby minimising the associated systematic uncertainties. The cross-section is measured to be: $\sigma_{t\bar{t}}$= 818 $\pm$ 8 (stat) $\pm$ 27 (syst) $\pm$ 19 (lumi) $\pm$ 12 (beam) pb, where the four uncertainties arise from data statistics, experimental and theoretical systematic effects, the integrated luminosity and the LHC beam energy, giving a total relative uncertainty of 4.4%. The result is consistent with theoretical QCD calculations at next-to-next-to-leading order. A fiducial measurement corresponding to the experimental acceptance of the leptons is also presented.

==> acknowledgements/Ackno-Bibtex_2Aug-2016.tex <==
% Acknowledgements for papers with collision data
% Version 2-Aug-2016

% Bibitem entry for the Tier2 facilities reference
%-------------------------------------------------
@Booklet{ATL-GEN-PUB-2016-002,
          author         = "{ATLAS Collaboration}",
          title          = "{ATLAS Computing Acknowledgements
      2016-2017}",
          howpublished   = "{ATL-GEN-PUB-2016-002}",
          url            = "http://cds.cern.ch/record/2202407",
          year           = "2016",
      } 
%----------------------------------------------



==> atlas-detector.tex <==
% Footnote with ATLAS coordinate system
\newcommand{\AtlasCoordFootnote}{%
ATLAS uses a right-handed coordinate system with its origin at the nominal interaction point (IP)
in the centre of the detector and the $z$-axis along the beam pipe.
The $x$-axis points from the IP to the centre of the LHC ring,
and the $y$-axis points upwards.
Cylindrical coordinates $(r,\phi)$ are used in the transverse plane, 
$\phi$ being the azimuthal angle around the $z$-axis.
The pseudorapidity is defined in terms of the polar angle $\theta$ as $\eta = -\ln \tan(\theta/2)$.
Angular distance is measured in units of $\Delta R \equiv \sqrt{(\Delta\eta)^{2} + (\Delta\phi)^{2}}$.}

%-------------------------------------------------------------------------------
\section{ATLAS detector}
\label{sec:atlas-detector}
%-------------------------------------------------------------------------------
The ATLAS detector~\cite{PERF-2007-01} at the LHC covers nearly the entire
solid angle around the collision point, and consists of an inner tracking
detector surrounded by a thin superconducting solenoid magnet producing
a 2\,T axial magnetic field, electromagnetic and hadronic calorimeters, and 
an external muon spectrometer incorporating three large toroid magnet 
assemblies. The inner detector consists of a high-granularity silicon pixel
detector, including the newly-installed insertable B-layer (IBL)~\cite{ibl}, 
and a silicon microstrip tracker, together providing precision
tracking in the pseudorapidity\footnote{ATLAS uses a right-handed coordinate 
system with its origin at
the nominal interaction point in the centre of the detector, and the $z$ axis
along the beam line. Pseudorapidity is defined in terms of the polar angle
$\theta$ as $\eta=-\ln\tan{\theta/2}$, and transverse momentum and energy
are defined relative to the beam line as $\pt=p\sin\theta$ and
$\et=E\sin\theta$. The azimuthal angle around the beam line is denoted by 
$\phi$, and distances in $(\eta,\phi)$ space by 
$\Delta R=\sqrt{\Delta\eta^2+\Delta\phi^2}$.} 
range $|\eta|<2.5$, complemented by a straw-tube transition radiation
tracker providing tracking and electron identification information for
$|\eta|<2.0$. A lead liquid-argon (LAr) electromagnetic calorimeter covers the
region $|\eta|<3.2$, and hadronic calorimetry is provided by 
steel/scintillating tile calorimeters for $|\eta|<1.7$ and copper/LAr
hadronic endcap calorimeters for $1.5< |\eta|<3.2$. The forward region is covered by additional
LAr calorimeters with copper and tungsten absorbers. The muon
spectrometer consists of precision tracking chambers covering the region
$|\eta|<2.7$, and separate trigger chambers covering $|\eta|<2.4$. 
A 
two-level trigger system, using custom hardware followed by a
software-based level, is used to reduce the event rate to a maximum of around 1\,kHz 
for offline storage.

%The ATLAS experiment~\cite{PERF-2007-01} at the LHC is a multi-purpose particle detector
%with a forward-backward symmetric cylindrical geometry and a near $4\pi$ coverage in 
%solid angle.\footnote{\AtlasCoordFootnote}
%It consists of an inner tracking detector surrounded by a thin superconducting solenoid
%providing a \SI{2}{\tesla} axial magnetic field, electromagnetic and hadron calorimeters, and a muon spectrometer.
%The inner tracking detector covers the pseudorapidity range $|\eta| < 2.5$.
%It consists of silicon pixel, silicon micro-strip, and transition radiation tracking detectors.
%Lead/liquid-argon (LAr) sampling calorimeters provide electromagnetic (EM) energy measurements
%with high granularity.
%A hadron (iron/scintillator-tile) calorimeter covers the central pseudorapidity range ($|\eta| < 1.7$).
%The end-cap and forward regions are instrumented with LAr calorimeters
%for both EM and hadronic energy measurements up to $|\eta| = 4.9$.
%The muon spectrometer surrounds the calorimeters and is based on
%three large air-core toroid superconducting magnets with eight coils each.
%Its bending power is in the range from \num{2.0} to \SI{7.5}{\tesla\metre}.
%It includes a system of precision tracking chambers and fast detectors for triggering.
%A three-level trigger system is used to select events.
%The first-level trigger is implemented in hardware and uses a subset of the detector information
%to reduce the accepted rate to at most \SI{75}{\kilo\hertz}.
%This is followed by two software-based trigger levels that
%together reduce the accepted event rate to \SI{400}{\hertz} on average
%depending on the data-taking conditions during 2012.



